In-situ amplification of spin echoes within a kinetic inductance parametric amplifier

The use of superconducting micro-resonators in combination with quantum-limited Josephson parametric amplifiers has in recent years lead to more than four orders of magnitude improvement in the sensitivity of pulsed Electron Spin Resonance (ESR) measurements. So far, the microwave resonators and amplifiers have been designed as separate components, largely due to the incompatibility of Josephson junction-based devices with even moderate magnetic fields. This has led to complex spectrometers that operate under strict environments, creating technical barriers for the widespread adoption of the technique. Here we circumvent this issue by inductively coupling an ensemble of spins directly to a weakly nonlinear microwave resonator, which is engineered from a magnetic field-resilient thin superconducting film. We perform pulsed ESR measurements with a $1$~pL effective mode volume and amplify the resulting spin signal using the same device, ultimately achieving a sensitivity of $2.8 \times 10^3$ spins in a single-shot Hahn echo measurement at a temperature of 400 mK. We demonstrate the combined functionalities at fields as large as 254~mT, highlighting the technique's potential for application under more conventional ESR operating conditions.

==> glossary.tex <==
% use \gls*{item} for a standard abbrev./acronym usage
% use \glspl*{item} for a plural usage, e.g. FPGAs
% use \acrshort*{item} to explicitly insert the acronym without expansion, recommended for figure captions which may appear before the main text.
%
%% Technical terms
\newacronym{cqed}{cQED}{circuit quantum electrodynamics}
\newacronym{cavqed}{CQED}{cavity quantum electrodynamics}
\newacronym{tl}{TL}{transmission line}
\newacronym{pbg}{PBG}{photonic bandgap}
\newacronym{lgr}{LGR}{loop-gap resonator}
\newacronym{esr}{ESR}{electron spin resonance}
\newacronym{nmr}{NMR}{nuclear magnetic resonance}
\newacronym{awg}{AWG}{arbitrary waveform generator}
\newacronym{pcb}{PCB}{printed circuit board}
\newacronym{cpw}{CPW}{coplanar waveguide}
\newacronym{rf}{RF}{radio-frequency}
\newacronym{mkid}{MKID}{microwave kinetic inductance detectors}
\newacronym{tls}{TLS}{two level system}
\newacronym{epr}{EPR}{electron paramagnetic resonance}
\newacronym{squid}{SQUID}{superconducting quantum interference device}
\newacronym{esd}{ESD}{electrostatic discharge}
\newacronym{sql}{SQL}{standard quantum limit}
\newacronym{snr}{SNR}{signal-to-noise ratio}
\newacronym{idc}{IDC}{interdigitated capacitor}
\newacronym{fid}{FID}{free induction decay}
\newacronym{em}{EM}{electromagnetic}
\newacronym{qho}{QHO}{quantum harmonic oscillator}
\newacronym{rms}{RMS}{root-mean-square}
\newacronym{bcs}{BCS}{Bardeen-Cooper-Schrieffer}
\newacronym{lpf}{LPF}{low-pass filter}
\newacronym{4wm}{4WM}{four wave mixing}
\newacronym{3wm}{3WM}{three wave mixing}
\newacronym{kipa}{KIPA}{kinetic inductance parametric amplifier}
\newacronym{jpa}{JPA}{Josephson parametric amplifier}
\newacronym{dpa}{DPA}{degenerate parametric amplifier}
\newacronym{cpmg}{CPMG}{Carr-Purcell-Meiboom-Gill}
\newacronym{lo}{LO}{local oscillator}



% Fab
\newacronym{sem}{SEM}{scanning electron microscope}
\newacronym{pmma}{PMMA}{poly(methyl methacrylate)}
\newacronym{nmp}{NMP}{N-Methyl-2-pyrrolidone}
\newacronym{hf}{HF}{hydrogen fluoride}
\newacronym{ebl}{EBL}{electron beam lithography}
\newacronym{rie}{RIE}{reactive ion etching}
\newacronym{fz}{FZ}{float-zone}
\newacronym{us}{US}{ultrasonicate}

%% Applications
\newacronym{mri}{MRI}{magnetic resonance imaging}
\newacronym{cmos}{CMOS}{complementary metal-oxide-semiconductor}
\newacronym{mos}{MOS}{metal-oxide-semiconductor}
\newacronym{rwa}{RWA}{rotating wave approximation}
\newacronym{nv}{NV}{nitrogen vacancy}
\newacronym{ivc}{IVC}{inner vacuum chamber}
\newacronym{vna}{VNA}{vector network analyzer}
\newacronym{smu}{SMU}{source measurement unit}
\newacronym{qip}{QIP}{quantum information processing}
\newacronym{hemt}{HEMT}{High Electron Mobility Transistor}

%% Companies
\newacronym{srs}{SRS}{Stanford Research Systems}
\newacronym{ni}{NI}{National Instruments}
\newacronym{cst}{CST}{Computer Simulation Technology}

%% Simulations and waves
\newacronym{fem}{FEM}{finite element method}
\newacronym{tem}{TEM}{transverse electromagnetic}


%%% regex for TLAs : \b[A-Z]{2}[A-Z]*\b
